Online Hyperparameter Meta-Learning with Hypergradient Distillation

Many gradient-based meta-learning methods assume a set of parameters that do not participate in inner-optimization, which can be considered as hyperparameters. Although such hyperparameters can be optimized using the existing gradient-based hyperparameter optimization (HO) methods, they suffer from the following issues. Unrolled differentiation methods do not scale well to high-dimensional hyperparameters or horizon length, Implicit Function Theorem (IFT) based methods are restrictive for online optimization, and short horizon approximations suffer from short horizon bias. In this work, we propose a novel HO method that can overcome these limitations, by approximating the second-order term with knowledge distillation. Specifically, we parameterize a single Jacobian-vector product (JVP) for each HO step and minimize the distance from the true second-order term. Our method allows online optimization and also is scalable to the hyperparameter dimension and the horizon length. We demonstrate the effectiveness of our method on two different meta-learning methods and three benchmark datasets.

==> approach.tex <==
\section{Approach}
In order to overcome the aforementioned limitations, we propose a novel algorithm that continuously approximates the response Jacobian in Eq.~\eqref{eq:unroll} by distilling its Jacobian-vector product into a computationally more efficient form. As a result, our method, which we name as \emph{HyperDistill}, requires to compute only a single Jacobian-vector product per each hypergradient step.
%Note that $1\leq h\leq H$ where we manually tune the maximum horizon $H$ in advance.


%Our algorithm is for online optimization, so each hypergradient is computed at any step $t=0,\dots,T-1$. Therefo    


\subsection{Knowledge distillation for online optimization}

We denote the current validation gradient by $\alpha_{t} = \frac{\partial \loss(w_{t},\lambda)}{\partial w_{t}}$ for $t=1,\dots,T$. 
%Further, since the vanilla RMD requires to store all the previous weights, we follow DrMAD~\cite{FuLFLC16} and linearly interpolate between $w_0$ and $w_{t}$ to get the approximations $\hat{w}_{1},\dots,\hat{w}_{t-1}$. As a result, we express the second-order term as follows:
We approximate the training Hessians with a scaled diagonal matrix. If we assume vanilla SGD, we have $A = \frac{\partial (w - \eta \grad \loss^\text{train}(w,\lambda))}{\partial w} = I - \eta \Lambda$, where $\eta$ is a learning rate and $\Lambda$ is a training Hessian. By letting $\Lambda \approx kI$, we have $A \approx (1-\eta k)I = \gamma I$.
\begin{align}
    \alpha_{t} \cdot \frac{\partial w_{t}}{\partial \lambda}\bigg|_{w_0} 
    = \sum_{i=1}^{t} \alpha_{t} A_t A_{t-1} \cdots A_{i+1} B_{i} \approx \sum_{i=1}^{t} \gamma^{t-i} \alpha_{t} B_{i}.
    \label{eq:unapproxiamted_so}
\end{align}
%where $\hat{A}_i = \frac{\partial \Phi(\hat{w}_{i-1}, \lambda; D  _i)}{\partial \hat{w}_{i-1}}$ and $\hat{B}_i = \frac{\partial \Phi(\hat{w}_{i-1}, \lambda; D_i)}{\partial \lambda}$.


%Our online optimization algorithm is based on $h$-step truncated unrolled differentiation~\cite{Shaban19truncated}. It means that for each online optimization step $t=1,\dots,T$, we will frequently need to iterate the $h$ previous steps $t-h+1,\dots,t$. To avoid cluttered notation, in this section we will suppress the notation $t$ throughout in the following way: steps $1,\dots,h$ in this section corresponds to the actual step $t-h+1,\dots,t$. Note that the horizon size $h$ can vary with $1 \leq h \leq H$, where we manually tune $H$. Based on those notations,

% \iffalse
% The first approximation is $\gamma^{h-i} \alpha_h \approx \alpha_h \prod_{j=i+1}^{h} \hat{A}_{j}$ for $0 \leq \gamma \leq 1$. The approximation is done by minimizing the Euclidean distance between them.
% \begin{align}
%     \gamma_* = \argmin_{\gamma} \left\| \gamma^{h} \alpha_h - \alpha_h \prod_{j=1}^{h} \hat{A}_{j} \right\| = \left( \frac{\langle \alpha_h, \alpha_h \hat{A}_1\cdots\hat{A}_h \rangle}{\langle \alpha_h, \alpha_h \rangle} \right)^{\frac{1}{h}}
% \end{align}
% %In addition, we empirically found that tracking the exact order of mini-batches $D_1,\dots,D_{h}$ has almost no effect to the convergence, both for DrMAD and our method. Thus, when we compute the hypergradient we simply sample the mini-batches again from the same batch-sampling distribution $p(D)$, which can be seen as the following approximation.
% Then, we have
% \begin{align}
%     \alpha_{h} \cdot \frac{\partial w_{h}}{\partial \lambda}\bigg|_{w_0} 
%     =
%     \alpha_{h} \sum_{i=1}^{h} \left( \prod_{j=i+1}^{h} A_{j}\right) B_{i}
%     = \sum_{i=1}^{h} c_{i}
%     \label{eq:approxiamted_so}
% \end{align}
% where we denote $c_{i} = \gamma_*^{h-i} \alpha_h \hat{B}_i$.
% \fi


%The difficulty of evaluating Eq.~\eqref{eq:unapproxiamted_so} with DrMAD is that we need to compute total $2t-1$ Jacobian-vector products. 
%The key idea is, what if we compute only a few of them and \emph{learn to approximate} Eq.~\eqref{eq:unapproxiamted_so} by those vectors? Towards this idea, we propose to project $c_1+c_2+\cdots+c_h$ onto the hyperplane formed by only the first term $c_1$ and the last term $c_h$. 
%Note that whereas the last term $c_h = \alpha_{h}\hat{B}_{h}$ has a computationally efficient form, the first term $c_1 = \alpha_{h} \hat{A}_h \hat{A}_{h-1} \cdots \hat{A}_{2} \hat{B}_{1}$ has a long chain of Jacobians. Therefore, 
%We firstly approximate as $A_i \approx \gamma I$ for all $i$. Specifically, we want
%\begin{align}
    %\alpha_t \hat{A}_t \hat{A}_{t-1} \cdots \hat{A}_{i+1} \hat{B}_i \approx \gamma^{t-i} %\alpha_t \hat{B}_i.
    %\label{eq:gamma}
%\end{align}
%for $\gamma > 0$. 
%We estimate $\gamma$ by minimizing the Euclidean distance between the two terms in Eq.~\eqref{eq:gamma}.
%\begin{align}
%    \gamma = \argmin_{\gamma} \left\| \gamma^{t} \alpha_t - \alpha_t \hat{A}_t \cdots \hat{A}_{1} \right\| = \left( \frac{\langle \alpha_t, \alpha_t \hat{A}_h\cdots\hat{A}_1 \rangle}{\langle \alpha_t, \alpha_t \rangle} \right)^{\frac{1}{t}}
%    \label{eq:gamma_solution}
%\end{align}

% Note that we do not compute Eq.~\eqref{eq:gamma_solution} for every hypergradient step but use the same $\gamma$ for a certain period, with the assumption that the training Hessian does not change too quickly. With $\gamma$ obtained from Eq.~\eqref{eq:gamma_solution}, the first term is approximated as $\hat{c}_1 = \gamma^{h-1} \alpha_h \hat{B}_1$, which can be computed by only a single Jacobian-vector product. Now we are ready to perform the projection. It is done by minimizing the Euclidean distance between the sum and the linear combination of $\hat{c}_1$ and $c_h$.
% \begin{align}
%     \min_{\pi} \left\|\pi_\text{first} \hat{c}_\text{1} + \pi_\text{last} c_h - \sum_{i=1}^{h} c_i \right\|
%     \label{eq:gamma_norm}
% \end{align}
% where $\pi = (\pi_\text{first}, \pi_\text{last})$ are the coefficients. Eq.~\eqref{eq:gamma_norm} has the following simple closed-form solution.
% \begin{align}
%     \pi = 
%     \left(\sum_{i=1}^h c_i\right) C^\top (C C^\top)^{-1},\quad\text{where}\quad C = \begin{bmatrix}\hat{c}_1 \\ c_h \end{bmatrix}
%     \label{eq:form_of_pi}
% \end{align}
% Again, we only periodically evaluate Eq.~\eqref{eq:form_of_pi} because computing the ground-truth $\sum_{i=1}^h c_i$ for every hypergradient step is computationally expensive. However, the difference from $\gamma$ is that it is not straightforward to capture the relationship between $\pi$ and the horizon size $h$, although $h$ is variable in online optimization setting. According to Eq.~\eqref{eq:form_of_pi}, $\pi_1$ and $\pi_h$ tend to be positively correlated with the horizon size $h$ if the directions of $c_1,c_2,\dots,c_h$ are not too different from each other. It means that we should estimate $\pi$ as a function of $h$ to make $\pi$ adaptive to each online optimization step.

\subsection{Proper form of $\pi^*$ as a function}

We next discuss how to obtain a proper form of $\pi^*$ as a function. In Eq.~\eqref{eq:form_of_pi}, the value of $\pi^*$ closely depends on how much the set of vectors $c_1,c_2,\dots,c_h$ are aligned to the same direction. Therefore, it is natural to think of Lipschitz continuity by viewing $c$ as a smooth function w.r.t some underlying variable $x$. Specifically, we define 
\[ c_t(w,D) = \alpha_t \frac{\partial \Phi (w,\lambda;D)}{\partial \lambda}. \] We assume that $\|c_t(w_i, D_i) - c_1\| \leq K \left\| x_{i} - x_1 \right\|_\mathcal{X}$ for all $i=1,\dots,h$ with a suitable metric $\|\cdot\|_\mathcal{X}$ and $K\geq 0$ the Lipschitz constant. The smaller the $K$, the greater the optimal $\pi_*$ will be. 

Knowledge distillation. For some $w$ and $D$,
\begin{align}
    \min_{\pi, w, D} \left\|\pi c_t(w,D) - \sum_{i=1}^{t} \gamma^{t-i} c_t(\hat{w}_{i-1}, D_i) \right\|, \quad \pi(w,D) = \frac{ \langle c_t(w,D), \sum_{i=1}^t \gamma^{t-i} c_t(w_{i-1},D_i) \rangle}{\langle c_t(w,D), c_t(w,D) \rangle}
    \label{eq:form_of_pi}
\end{align}

Following this intuition, we propose to capture the functional form of $\pi_*$ from the upper bound of the Lipschitz inequality. Recall from Eq.~\eqref{eq:approxiamted_so} that the function $c$ is written as follows:
\begin{align}
    c(i, D_i\ ;\ h,w_0,w_h,\lambda,\alpha_h,\gamma_*) = \gamma_*^{h-i} \alpha_h
    \frac{\partial \Phi(\hat{w}_i,\lambda;D_i)}{\partial \lambda}.
    \label{eq:cfunction}
\end{align}
Therefore, the index $i$ and the current mini-batch $D_i$ are the two underlying variables when the othter factors $h$, $w_0$, $w_h$, $\lambda$, $\alpha_h$, and $\gamma_*$ are given. Note that all the weight interpolations $\hat{w}_j = (1-\frac{j}{h})w_0 + \frac{j}{h}w_h$ for $j=i,\dots,h-1$ are fully specified when $h$, $w_0$, and $w_h$ are given. Now we apply the Lipschitz continuity assumption. 
\begin{align}
    0 \leq \|c_{i} - c_1\| \leq K \left\| (i, D_i) - (1, D_1) \right\|_\mathcal{X},\quad\text{for}\quad i = 1,\dots,h.
    \label{eq:lipschitz}
\end{align} 
We let the metric $\|\cdot\|_\mathcal{X}$ appropriately scale each input element, such that we conveniently define $K^2\|(i,D)\|_\mathcal{X} = K_1\|i\|^2 + K_2\|D\|^2$. Based on them, we can readily derive the following theorem.
\begin{thm}
\label{thm:1}
    Suppose Eq.~\eqref{eq:lipschitz} holds with $K_1,K_2 \geq 0$. Further suppose for $i=0,\dots,h-1$ that $1-\delta \leq \|c_{i}\|^2 / \|c_0\|^2 \leq 1+\delta$ with a sufficiently small $\delta > 0$. Then, we have
    \begin{align}
    \left(1-\frac{\delta}{2} - \frac{K_2 Q}{2\|c_1\|^2} \right)h - \frac{K_1}{2 \|c_1\|^2} f(h) \leq \pi_* \leq 
    \left(1 + \frac{\delta}{2}\right)h
    \label{eq:thm}
    \end{align}
    where $f(h) = \sum_{i=0}^{h-1}i = h(h-1)(2h-1)/6$. Proof in \textbf{the supplementary file}.
\end{thm}

The lower bound of Eq.~\eqref{eq:thm} corresponds to the upper bound of Eq.~\eqref{eq:lipschitz}. We see from the lower bound that whereas the first term is positively correlated with $h$ as expected, the second term quickly deteriorates the lower bound as $h$ increases, which means that we need to carefully set the horizon size $h$. This agrees with our empirical observation that $h$ can maximally increase to $10$ or $15$, but longer $h$ gradually decreases the value of $\pi^*$. For $Q$, it tells that we need to measure how far the current batch $D_1$ is from the batch mean. It may be done by accumulating the batch mean and measure the distance between $D_1$ and the mean.
However, in this work we do not condition $\pi^*$ on $D_1$ for simplicity and leave it as a future work.


\begin{figure}[t]
    \begin{minipage}[t]{.5\textwidth}
    \begin{algorithm}[H]
    	\caption{$\beta$ Estimation}\label{alg:beta}
    	\small
    	\begin{algorithmic}[1]
    		\State \textbf{Input:} The current weight $w_{t+h}$, the previous weight $w_t$, and the current validation gradient $\alpha_{t+h}$.
    		\State \textbf{Output:} Estimated $\gamma$.
    		\State $b_\text{sum} \leftarrow 0$
    		\State$X = [\ ], y = [\ ]$
    		\For{$i=h-1$ \textbf{downto} $0$}
    		\State $\hat{w}_{t+i} \leftarrow \left(1-\frac{i}{h}\right) w_t + \frac{i}{h} w_{t+h}$
    		\State $r \leftarrow \|w_{t+h}-\hat{w}_{t+i}\|^2/\|b_{t+i}\|^2$
    		\State $h' \leftarrow h-i$
    		\State $X \leftarrow X.\text{concat}((h', h'r, r))$ 
    		\State $b \leftarrow \alpha_{t+h}\hat{B}_{t+i}$
    		\State $b_\text{sum} \leftarrow b_\text{sum} + b$
    		\State $\pi^* \leftarrow b \tran b_\text{sum} / b \tran b$
    		\State $y \leftarrow y.\text{concat}(\pi^*)$
    		\EndFor
    		\State $\gamma \leftarrow \text{LinearRegression}(X,y)$ \\
    		\Return $\gamma$
    	\end{algorithmic}
    	\end{algorithm}
    \end{minipage}
    \begin{minipage}[t]{.5\textwidth}
    \begin{algorithm}[H]
    	\caption{Meta-training}
    	\small
    	\begin{algorithmic}[1]
    		\State \textbf{Input:} The last state $s_T$ and the initial state $s_0$.
    		\State \textbf{Output:} Approximated hyper-gradient $g$.
    		\State $\alpha \leftarrow\frac{\partial \tilde\loss(s_T,\lambda)}{\partial s_T},\quad g \leftarrow \frac{\partial \tilde\loss(s_T,\lambda)}{\partial \lambda}$
    		\For{$t=T-1$ \textbf{downto} $0$}
    		\State $\hat{s}_t \leftarrow \left(1-\frac{t}{T}\right) s_0 + \frac{t}{T} s_T$
    		\State $g \leftarrow g + \alpha\hat{B}_{t+1}$
    		\State $\alpha \leftarrow \alpha \hat{A}_{t+1}$
    		\EndFor \\
    		\Return $g$
    	\end{algorithmic}
    	\end{algorithm}
    \end{minipage}
\end{figure}
%, that is, we regard $Q$ as a constant shared over all the cases. It will be also interesting to see if can tighten the lower bound by distilling the whole dataset into $D_0^*$.
%However, since it is not straightforward to measure the distance between a set of raw batches, here we treat the average distance as a constant $Q$ for simplicity.

\subsection{Constructing a function estimator}
We estimate the function with a small neural network. 
\begin{align}
    \hat{\pi}_\text{first}(h), \hat{\pi}_\text{last}(h) = \nn(h;\theta)
    \label{eq:estimator}
\end{align}
where $\hat{\pi}_\text{first}(h)$ and $\hat{\pi}_\text{last}(h)$ are the estimations and $\nn(h;\theta)$ is a neural network parameterized by $\theta$.d In order to learn this network we need to collect samples of $(h,\pi)$ and iteratively perform the optimization. We propose to collect the samples from DrMAD procedure in Algorithm~\ref{alg:drmad}, where at the end of every \textbf{for} iteration we can set the horizon size to $h = T-i$ and the corresponding scaler to $\pi = c \tran g / c \tran c$ with $c = \alpha\hat{B}_i$. Note that we can efficiently collect all the inputs and targets from only a single backward travel through the interpolated weights. See Algorithm~\ref{alg:beta} for the detailed procedure.

\vspace{-0.05in}
\paragraph{Periodic re-estimation} Note that the form of the function $c$ in Eq.~\eqref{eq:cfunction} depends on other factors than $h$ as well, such as the initial weight $w_0$, the last weight $w_h$, the hyperparameter $\lambda$, the validation gradient $\alpha_{h}$, and the Hessian decaying factor $\gamma_*$. Although less significant than $h$, the lower bound of Eq.~\eqref{eq:thm} also depends on them through $K$, $\delta$ and $\|c_0\|$. As they gradually change as we proceed meta-training, we periodically re-estimate the decaying factor $\gamma_{*}^\text{new}$ and the parameter $\beta^\text{new}$ through the Algorithm~\ref{alg:beta} and update with the exponential moving average: $\gamma_* \leftarrow \mu \gamma_* + (1-\mu)\gamma_*^\text{new}$ and $\beta \leftarrow \mu \beta + (1-\mu) \beta^\text{new}$. We used $\mu=0.5$ in our experiments. We empirically found that very sparse period works well, for instance every $20$ inner-optimizations. It suggests that the variations in those factors do not chaotically affect $\gamma_*$ and $\pi_*$, allowing our estimator $\hat{\pi}_*(\cdot;\beta)$ in Eq.~\eqref{eq:estimator} to remain stable and computationally efficient during the entire meta-training process.

% \subsection{Extending the horizon size}
% %The lower bound of Eq.~\eqref{eq:thm} tells that there is a limitation with which we can increase the horizon size $h$. Therefore, 
% Applying our approximation to only a single horizon may not be enough to alleviate the short horizon bias. We thus propose to extend the horizon size by concatenating a few horizons one after the other. When the current step $h$ is $1 \leq h \leq H$, we approximate with $c_1 + c_2 + \cdots + c_h \approx \hat{\pi}_\text{first}(h)\hat{c}_1 + \hat{\pi}_\text{last}(h) c_h$. When $H < h \leq 2H$, we have
% \begin{align}
%     \sum_{i=1}^{H} c_{i} + \sum_{i=H+1}^{h} c_i 
%     \approx \big(\hat{\pi}_\text{first}(H) \hat{c}_1 + \hat{\pi}_\text{last}(H) \hat{c}_{H}\big) + \big(\hat{\pi}_\text{first}(h-H) \hat{c}_{H+1} + \hat{\pi}_\text{last}(h-H) c_{h}\big)
%     \label{eq:concat}
% \end{align}
% where $\hat{c}_1 = \gamma^{h} \alpha_h \hat{B}_1$, $\hat{c}_{H} = \gamma^{h-H+1} \alpha_h \hat{B}_{H}$, $\hat{c}_{H+1} = \gamma^{h-H} \alpha_h \hat{B}_{H+1}$, and $c_{h} = \alpha_h \hat{B}_{h}$. Applying $\alpha_h \hat{B}_H \approx \alpha_h \hat{B}_{H+1}$, we have
% \begin{equation}
% \begin{aligned}
% c_1 + c_2 + \cdots + c_h &\approx \hat{\pi}_\text{first}(H) \gamma^h {\color{red}\alpha_h \hat{B}_1}  \\
% &\quad+ \big(\hat{\pi}_\text{last}(H) \gamma^{h-H+1} + \hat{\pi}_\text{first}(h-H)\gamma^{h-H}\big) {\color{red}\alpha_h \hat{B}_H} \\
% &\quad+ \hat{\pi}_\text{last}(h-H) {\color{red}\alpha_h \hat{B}_h}.
% \end{aligned}
% \end{equation}
% Therefore, we only need to compute the three Jacobian-vector products, $\alpha_h \hat{B}_1$, $\alpha_h \hat{B}_H$, and $\alpha_h \hat{B}_h$ to cover the horizon of maximum $2H$ steps. It is straightforward to generalize to more than two horizons, and we only need to compute $n$ Jacobian-vector products to cover $(n-1)H$ steps. In our experiments, we set $H=10$ and concatenate only two horizons.


\iffalse
\subsection{Function approximation}

Suppose that $s_{t}$ is constant w.r.t $\lambda$ and we are interested in approximating the hyper-gradient over the next $h$ gradient steps. We propose the following approximation.
\begin{align}
    \frac{\partial s_{t+h}}{\partial \lambda}\bigg|_{s_t} \approx \pi(\|s_{t+h}-s_t\|_2) \cdot \frac{\partial s_{t+1}}{\partial \lambda}\bigg|_{s_t}
\end{align}
where $\pi: \mathbb{R} \rightarrow [1,\infty)$. In other words, we have
\begin{align}
     \frac{\partial \Phi_{t+h}(\cdots \Phi_{t+1}(s_{t},\lambda),\cdots,\lambda)}{\partial \lambda} 
     \approx 
     \pi(\|s_{t+h}-s_t\|_2) \cdot \frac{\partial \Phi_{t+1}(s_{t},\lambda)}{\partial \lambda}
\end{align}
The intuition is that
\fi

%\begin{align}
%    h - \frac{h}{2}\delta - K^2 \frac{(h-1)(2h-1)}{12h} \frac{\|s_h - s_0\|^2}{\|a_0\|^2} - C \leq %\pi^* \leq h + \frac{h}{2}\delta
%\end{align}
%for a sufficiently small $\delta > 0$ and $t=0,\dots,h-1$. We need to make the lower bound as tight as possible by finding the best possible Lipschitz constant $K$. Define $g_h := \|s_h-s_0\|^2 / \|a_0\|^2$ Then, the lower bound $L(\pi^*)$ is given as

%By taking square on those inequalities and taking sum over $t=0,\dots,h-1$, we have
%\begin{align}
%    0 \leq \sum_{t=0}^{h-1} \|a_0 - a_t\|^2 \leq K^2 \sum_{t=0}^{h-1} \|s_0-s_t\|^2 + K^2 \sum_{t=0}^{h-1}\|D_0-D_t\|^2 
%\end{align}
%Rearranging the terms, we can show that
